Tri-Cam: Practical Eye Gaze Tracking via Camera Network

As human eyes serve as conduits of rich information, unveiling emotions, intentions, and even aspects of an individual's health and overall well-being, gaze tracking also enables various human-computer interaction applications, as well as insights in psychological and medical research. However, existing gaze tracking solutions fall short at handling free user movement, and also require laborious user effort in system calibration. We introduce Tri-Cam, a practical deep learning-based gaze tracking system using three affordable RGB webcams. It features a split network structure for efficient training, as well as designated network designs to handle the separated gaze tracking tasks. Tri-Cam is also equipped with an implicit calibration module, which makes use of mouse click opportunities to reduce calibration overhead on the user's end. We evaluate Tri-Cam against Tobii, the state-of-the-art commercial eye tracker, achieving comparable accuracy, while supporting a wider free movement area. In conclusion, Tri-Cam provides a user-friendly, affordable, and robust gaze tracking solution that could practically enable various applications.

==> discussion.tex <==
\section{Discussion}

% \subsection{Tri-Cam Can Also be Deployed on Laptop}

% In the experiment, we mainly deployed Tri-Cam on the Dell 27'' monitor.
% Although we also deployed and tested Tri-Cam on the 18'' Alienware laptop monitor, laptops do have some issue with webcam deployment.
% Laptops 

\subsection{Better Eye Detection Design}

In this work, our primary focus is on the gaze tracking task, and we have simply adopted the Mediapipe algorithm for eye detection. The Mediapipe algorithm initially detects the human face and then utilizes it as a reference to locate the eyes, which proves to be more robust compared to direct eye detection algorithms like the OpenCV package. However, the eye detection module consistently outputs cropped eye images regardless of whether the eyes are open or closed. Consequently, numerous low-quality eye images are incorporated into the data pool for both training and testing, even though it would be valid to pause the eye tracking task in instances of closed or barely visible eyes. Although the weighted fusion module partially mitigates the impact of low-quality images, it would be advantageous to filter the eye images before their utilization in training or testing to further enhance gaze tracking performance. However, we have not extensively addressed or designed solutions for this issue, as our primary focus in this work is on the gaze tracking task itself. If Tri-Cam is to be potentially applied in real-world scenarios, improving the eye detection module and refining data quality should be relatively feasible. We leave this aspect to be explored in future works.


\subsection{Better Implicit Data Collection Strategy}

We only developed simple and deterministic criteria for the implicit re-calibration module, utilizing application context, press-release duration, and screen-based location to filter collected click opportunities. While this approach allowed clicks with high alignment error into the data pool and potentially discarded accurate clicks, it was due to the simplicity of the strategies employed.

We believe that incorporating more detailed context information holds promise for enhancing both the quality and efficiency of implicit data collection. For instance, if the data collection module could access the location of all interaction buttons in an active window, we could prioritize these areas to assess click quality. Furthermore, the size of buttons could impact click accuracy; smaller buttons necessitate more precise attention from users, likely leading to higher click accuracy. However, accessing such detailed context information may raise privacy concerns.

Moreover, we only enlisted five users to collect real-life computer usage data, as it proved to be rather expensive. Participants had to sit in front of a designated monitor with webcams positioned on top, and the Tobii Pro Spark eye tracker in operation. However, the high-frequency-strobing infrared emitter of the Tobii Pro Spark eye tracker, as reported by three of the participants, caused eye discomfort after prolonged exposure. This prompts us to consider replacing or bypassing the Tobii Pro Spark in future studies. For example, we may explore training the model directly using implicitly collected data and evaluating its accuracy as an indicator of data quality.
However, this approach would inevitably increase the burden of research.

Additionally, participants' behavior may differ from their real-life habits when asked to participate in a computer usage study, further complicating data collection. Nonetheless, we remain interested in researching implicit re-calibration in the future, as it holds the potential to reduce or eliminate gaze data collection overhead.



==> related.tex <==
\section{Related Work}

Eye gaze tracking receives considerable research interest owing to its diverse applications in human-computer interaction \cite{duchowski2007eye, majaranta2014eye, salvucci2000identifying, borji2014defending, holmqvist2011eye}, psychology \cite{liversedge2000saccadic, hessels2019eye, holmqvist2017eye}, medicine \cite{borji2014defending, wu2008detecting, pfeiffer2013gaze, vrij2000detecting}, and beyond.
Several recent studies have explored innovative applications of eye gaze tracking technology in interactive systems and wearable devices. 
Khamis et al. introduced GazeTouchPIN, a multimodal authentication system designed to safeguard sensitive data on mobile devices by integrating gaze input and touch interaction \cite{huang2018gazetouchpin}. 
Jansen et al. presented EyeScout, a system for active eye tracking facilitating position-independent gaze interaction with large public displays \cite{jansen2014eyescout}. 
% In this section, we review existing literature on eye gaze tracking, focusing on two prominent approaches: geometric and deep learning-based gaze tracking.

% \subsection{geometric Gaze Tracking}

As a basic way of gaze tracking, geometric methods leverage the geometric relationships between the eye and a camera or sensor to estimate the direction of gaze \cite{holmqvist2011eye,duchowski2007eye,chamberlain2007eye}. 
These methods often rely on precise calibration procedures and mathematical models to infer gaze direction accurately .
Early geometric gaze tracking techniques, such as the corneal reflection method \cite{holmqvist2011eye}, utilized the reflection of light on the cornea and pupil to estimate gaze direction \cite{duchowski2007eye,chamberlain2007eye}. 
By analyzing the positions of corneal reflections relative to known features in the eye or environment, researchers were able to determine the direction of gaze with reasonable accuracy. 
However, these methods often required controlled lighting conditions and were sensitive to head movements.

Recent advancements in geometric gaze tracking have led to the development of non-invasive, camera-based systems that can accurately estimate gaze direction in real-time. 
Techniques such as model-based tracking, where 3D models of the eye and surrounding features are used to infer gaze direction, have shown decent results in improving accuracy and robustness \cite{majaranta2014eye}.
Another recent work, AS-Gaze\cite{ASgaze} uses iris model to estimate the gaze ray, and can be configured to track gaze points on various surfaces, such as mobile phone screens, computer displays or even whiteboards.
However, As-Gaze is likely unable to support free-movement.
It uses only a single camera, and does not discuss how to acquire the depth information.
Additionally, mathematically matching a ellipse with iris boundary and infer gaze point takes long time, thus As-Gaze is only able to support 11Hz inference, which is not enough for real time applications.
% One example is the use of multiple cameras or infrared sensors to capture stereo images of the eye, allowing for more robust and accurate gaze estimation. 
% Additionally, 

% Despite these advancements, geometric gaze tracking methods still face challenges in dealing with occlusions, variations in lighting conditions, and individual differences in eye morphology \cite{holmqvist2011eye}. 
% Moreover, the need for precise calibration and specialized hardware can limit their practicality in certain applications.

% \subsection{Deep Learning-Based Gaze Tracking}

Many gaze tracking works seek solution in deep learning method \cite{Balim_2023_CVPR, DVgaze, park2020eve}, as a most recent one that uses multiple cameras to estimate gaze point, DV-Gaze is able to handle free-movement using its double camera to perceive depth.
DV-Gaze uses both Resnet \cite{resnet} to process face image, and also uses Transformer \cite{transformer} to encode the camera calibration result, so that the network is capable of handling geometric relationship between cameras.
However, both components are computationally intensive, and do not fit practical application scenario, especially given that DV-Gaze uses face image which can be larger and more complex than eye images.
Therefore the training overhead of DV-Gaze is heavy, potentially making it hard to be practically deployed.
% While deep learning-based gaze tracking has shown remarkable performance improvements over traditional methods, it is not without its challenges. 
% One of the main limitations is the requirement for large amounts of labeled data for training, which can be costly and time-consuming to collect. 
% Moreover, deep learning models may struggle with generalization to unseen environments or individuals, requiring careful validation and fine-tuning.






